DeepProcess: Supporting business process execution using a MANN-based recommender system

Process-aware Recommender systems can provide critical decision support functionality to aid business process execution by recommending what actions to take next. Based on recent advances in the field of deep learning, we present a novel memory-augmented neural network (MANN) based approach for constructing a process-aware recommender system. We propose a novel network architecture, namely Write-Protected Dual Controller Memory-Augmented Neural Network (DCw-MANN), for building prescriptive models. To evaluate the feasibility and usefulness of our approach, we consider three real-world datasets and show that our approach leads to better performance on several baselines for the task of suffix recommendation and next task prediction.

==> extra.tex <==


%Process-aware Recommender Systems have been proposed to assist process owners in operational decision-making by recommending paths of a running instance that lead to good outcomes, up to its completion 

%Such recommendations are context-aware, adaptable, and focus on decisions like what task to execute next or enhance resource allocation policies and so on  \cite{schonenberg2008supporting}.

%This is made possible by Prescriptive process monitoring techniques that monitor process instances, and  consider the impact on the process performance to learn and predict future states and recommend appropriate actions.   


%can be used to directly support managers, stakeholders and process users in %, where goalsupporting activities or resources are recommended as the pre-defined goal
%optimization Our work differs in two ways i)we consider the problem of path recommendation



%In \cite{tax2017predictive} Tax et al. show that LSTMs can outperform existing methods for various prediction tasks such as next event prediction and associated timestamp predictions. The authors argue that compared to traditional methods LSTMs are task and dataset agnostic and do not require careful tuning and `trial-and-error' methodology for achieving good results. Similarly, Evermann et al. \cite{evermann2017predicting} and Navarin etl al \cite{navarin2017lstm} solve the same problem using recurrent neural networks and LSTMs respectively. They both perform evaluation on real-world datasets, for example using BPI2012 and BPI2013 datasets and achieve better results compared to the traditional approaches, thus providing evidence that deep learning methods are good at learning generalised representations even from noisy raw data usually found in event logs.



%Breuker et al. \cite{breuker2016comprehensible} for example employ probabilistic modelling(Inspired from the work done in the field of grammatical inference). A Drawback of their technique is that its computationally very intensive and the runtime reported by the authors was two months making it unsuitable for most practical industry applications. In \cite{ceci2014completion} pattern miner the frequent partial processes are identified first. The miner represents them in the sequence tree form while mapping each node of the tree to some specific prediction model trained using events logs,. After the training is done these models can be used for various prediction tasks such as next activity prediction or completion time of a process instance.

%Lakshmanan et al. \cite{lakshmanan2015markov} employ markov chains to estimate the instance-specific probabilistic process model (PPM) that can take as input a running process instance and compute probability of execution of a particular task in that instance. Similarly, Le et al. \cite{le2012hybrid} propose methods which use sequential k-nearest neighbour and higher order Markov models for predicting next process tasks. Lastly Polato et al. present methods for Time and Activity Sequence Prediction that tackle both stationary and dynamic(non-stationary) processes.



%\begin{enumerate}
%\item Is this overkill to use very complex model for relatively simple process
%analytics task?
%\item What are the implication for future predictive and prescriptive business
%modeling?
%\item Can plug-and-play style the end of domain knowledge in BPM? Can we
%just collect the whole lot amount of data and let the black-box model
%run?
%\end{enumerate}
%\subsection{Conclusion}

